Joint Resource Allocation and Transceiver Design for Sum-Rate Maximization under Latency Constraints in Multicell MU-MIMO Systems

Due to the continuous advancements of orthogonal frequency division multiplexing (OFDM) and multiple antenna techniques, multiuser multiple input multiple output (MU-MIMO) OFDM is a key enabler of both fourth and fifth generation networks. In this paper, we consider the problem of weighted sum-rate maximization under latency constraints in finite buffer multicell MU-MIMO OFDM systems. Unlike previous works, the optimization variables include the transceiver beamforming vectors, the scheduled packet size and the resources in the frequency and power domains. This problem is motivated by the observation that multicell MU-MIMO OFDM systems serve multiple quality of service classes and the system performance depends critically on both the transceiver design and the scheduling algorithm. Since this problem is non-convex, we resort to the max-plus queuing method and successive convex approximation. We propose both centralized and decentralized solutions, in which practical design aspects, such as signaling overhead, are considered. Finally, we compare the proposed framework with state-of-the-art algorithms in relevant scenarios, assuming a realistic channel model with space, frequency and time correlations. Numerical results indicate that our design provides significant gains over designs based on the wide-spread saturated buffers assumption, while also outperforming algorithms that consider a finite-buffer model.

==> 6 - Final Version/acronyms.tex <==
% !TeX root = manuscript.tex
% !TeX spellcheck = en_US

\acro{1G}{first generation}
\acro{2G}{second generation}
\acro{3G}{third generation}
\acro{4G}{fourth generation}
\acro{5G}{fifth generation}
\acro{5G-StoRM}{5G stochastic radio channel for dual mobility}
\acro{3GPP}{3rd Generation Partnership Project}
\acro{3GPP2}{3rd Generation Partnership Project 2}
\acro{ADMM}{alternating direction method of multipliers}
\acro{BB}{branch and bound}
\acro{BER}{bit error rate}
\acro{BS}{base station}
\acro{CDF}{cumulative distribution function}
\acro{CSI}{channel state information}
\acro{CFN}{channel Frobenius norm}
\acro{DPC}{dirty paper coding}
\acro{DCP}{difference of convex functions program}
\acro{GTEL}{Wireless Telecommunications Research Group}
\acro{GUB}{global upper bound}
\acro{GLB}{global lower bound}
\acro{HMSINR}{highest minimum \ac{SINR}}
\acro{HWCR}{highest \ac{WCR}}
\acro{HWSR}{highest weighted sum rate}
\acro{IBC}{interference broadcast channel}
\acro{IC}{interference channel}
\acro{ITS}{intelligent transport system}
\acro{JSFRA}{joint space-frequency
	resource allocation}
\acro{KKT}{Karush-Kuhn-Tucker}
\acro{LB}{lower bound}
\acro{LOS}{line of sight}
\acro{LP}{linear programming}
\acro{MILP}{mixed integer linear programming}
\acro{MIMO}{multiple input multiple output}
\acro{MINLP}{mixed integer nonlinear programming}
\acro{MIP}{mixed integer programming}
\acro{MISO}{multiple input single output}
\acro{MM}{majorization-minimization}
\acro{MMSE}{minimum mean squared error}
\acro{MRC}{maximum ratio combining}
\acro{MRT}{maximum ratio transmission}
\acro{MSE}{mean squared error}
\acro{MU-MIMO}{multi-user multiple input multiple output}
\acro{MU}{multi-user}
\acro{OFDM}{orthogonal frequency division multiplexing}
\acro{NLP}{nonlinear programming}
\acro{NLOS}{non-line of sight}
\acro{NP}{non-polynomial time}
\acro{PDF}{probability density function}
\acro{RRV}{rate-relaxation variable}
\acro{RUE}{resource usage efficiency}
\acro{QoS}{quality of service}
\acro{SCA}{successive convex approximation}
\acro{SCM}{stochastic channel model}
\acro{SINR}{signal to interference-plus-noise ratio}
\acro{SISO}{single input single output}
\acro{SIMO}{single input multiple output}
\acro{SNR}{Signal to Noise Ratio}
\acro{SOCP}{second-order cone programming}
\acro{TTI}{transmission time interval}
\acro{TU}{typical urban}
\acro{UE}{user equipment}
\acro{UB}{upper bound}
\acro{ULA}{uniform linear array}
\acro{UMi}{urban micro}
\acro{V2X}{vehicle-to-everything}
\acro{WINNER}{Wireless World Initiative New Radio}
\acro{WMMSE}{weighted minimum mean squared error}
\acro{WCR}{weighted common rate}
\acro{WP}{work package}
\acro{ZF}{zero-forcing}
\acro{ZMCSCG}{Zero Mean Circularly Symmetric Complex Gaussian}


==> 6 - Final Version/math.tex <==
%%%%%%%%%%%%%%%%
%% Math stuff %%
%%%%%%%%%%%%%%%%

% Alphabets (new fonts)
\DeclareMathAlphabet{\mathppl}{T1}{ppl}{m}{it}
\DeclareMathAlphabet{\mathphv}{T1}{phv}{m}{it}
\DeclareMathAlphabet{\mathpzc}{T1}{pzc}{m}{it}
% Operators
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\blockdiag}{blockdiag}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\subto}{\text{s.t.: }}
\DeclareMathOperator{\SubTo}{\text{subject to: }}
\DeclareMathOperator{\Vect}{vec}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\nullity}{nullity}
% Commands
\newcommand{\ArgMaxMin}[2]{\underset{#1}{\arg\max\min}\left\{#2\right\}}
\newcommand{\ArgMax}[2]{\underset{#1}{\arg\max}\left\{#2\right\}}
\newcommand{\ArgMinMax}[2]{\underset{#1}{\arg\min\max}\left\{#2\right\}}
\newcommand{\ArgMin}[2]{\underset{#1}{\arg\min}\left\{#2\right\}}
% Requires 'mathtools' package
% http://tex.stackexchange.com/questions/19431/how-to-write-a-limit-and-how-to-use-large-absolute-value
% \Abs{}       : same as \lvert{}\rvert
% \Abs[\Big]{} : same as \Bigl\vert{}\Bigr\vert
% \Abs*{}      : same as \left\vert{}\right\vert
%\DeclarePairedDelimiter\defAbs{\lvert}{\rvert}
%\newcommand{\Abs}[1]{\defAbs[\big]{#1}}
%\DeclarePairedDelimiter\Abs{\lvert}{\rvert}
%\newcommand{\Abs}[1]{\left\vert #1 \right\vert}
%\newcommand{\Abs}[1]{\vert #1 \vert}
\newcommand{\Adj}[1]{\adj\left( #1 \right)}
\newcommand{\Avg}[1]{\overline{#1}}
%\newcommand{\Card}[1]{\card\left\{#1\right\}}
\newcommand{\Card}[1]{\##1}
\newcommand{\Ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\Conj}[1]{{#1}^*}
\newcommand{\Cos}[1]{\cos\left( #1 \right)}
\newcommand{\Det}[1]{\det\left(#1\right)}
\newcommand{\Diag}[1]{\mathcal{D}\left\{ #1 \right\}}
\newcommand{\Elem}[2]{\left[{#1}\right]_{#2}}
\newcommand{\Exp}[1]{\text{e}^{#1}}
\newcommand{\Field}[1]{\mathbb{\uppercase{#1}}}
\newcommand{\First}{1^{\text{st}}}
\newcommand{\Floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\Herm}[1]{{#1}^{\mathrm{H}}}
\newcommand{\HInv}[1]{{#1}^{-\mathrm{H}}}
\newcommand{\InnerProd}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\Inv}[1]{{#1}^{-1}}
\newcommand{\TInv}[1]{{#1}^{-\mathrm{T}}}
\newcommand{\Lagrange}{\calL}
\newcommand{\LogTen}{\log_{10}}
\newcommand{\LogTwo}{\log_{2}}
\newcommand{\Max}[1]{\max\left\{ #1 \right\}}
\newcommand{\Mean}[1]{\mathcal{E}\left\{ #1 \right\}}
\newcommand{\Min}[1]{\min\left( #1 \right)}
\newcommand{\Mod}[1]{\left\vert #1 \right\vert}
\newcommand{\MOD}[1]{\vert #1 \vert}
\newcommand{\Mt}[1]{\mathbf{#1}}
\newcommand{\MtS}[1]{\boldsymbol{#1}}
\newcommand{\Norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\NormF}[1]{\Norm{#1}_{\mathrm{F}}}
\newcommand{\NormInf}[1]{\Norm{#1}_{\infty}}
\newcommand{\NormOne}[1]{\Norm{#1}_{1}}
\newcommand{\NormP}[1]{\Norm{#1}_{p}}
\newcommand{\NormTwo}[1]{\Norm{#1}_{2}}
\newcommand{\NORM}[1]{\Vert #1 \Vert}
\newcommand{\NORMF}[1]{\NORM{#1}_{\mathrm{F}}}
\newcommand{\NORMINF}[1]{\NORM{#1}_{\infty}}
\newcommand{\NORMONE}[1]{\NORM{#1}_{1}}
\newcommand{\NORMP}[1]{\NORM{#1}_{\text{p}}}
\newcommand{\NORMTWO}[1]{\NORM{#1}_{2}}
\newcommand{\Null}[1]{\calN\left(#1\right)}
\newcommand{\Nullity}[1]{\nullity\left(#1\right)}
\newcommand{\Order}[1]{\mathcal{O}\!\left(#1\right)}
\newcommand{\Ord}[1]{{#1}^{\text{th}}}
\newcommand{\PInv}[1]{{#1}^{\dagger}}
\newcommand{\Range}[1]{\calR\left(#1\right)}
\newcommand{\Rank}[1]{\rank\left(#1\right)}
\newcommand{\Real}[1]{\re\left\{#1\right\}}
\newcommand{\Round}[1]{\left\lceil #1 \right\rfloor}
\newcommand{\Set}[1]{\mathcal{\uppercase{#1}}}
\newcommand{\Second}{2^{\text{nd}}}
\newcommand{\Sin}[1]{\sin\left( #1 \right)}
\newcommand{\Third}{3^{\text{rd}}}
\newcommand{\Trace}[1]{\tr\left(#1\right)}
\newcommand{\Transp}[1]{{#1}^{\mathrm{T}}}
\newcommand{\Vector}[1]{\Vect\left\{#1\right\}}
\newcommand{\Vt}[1]{\mathbf{\lowercase{#1}}}
% Matrices
\newcommand{\mtA}{\Mt{A}}
\newcommand{\mtB}{\Mt{B}}
\newcommand{\mtC}{\Mt{C}}
\newcommand{\mtD}{\Mt{D}}
\newcommand{\mtE}{\Mt{E}}
\newcommand{\mtF}{\Mt{F}}
\newcommand{\mtG}{\Mt{G}}
\newcommand{\mtH}{\Mt{H}}
\newcommand{\mtI}{\Mt{I}}
\newcommand{\mtJ}{\Mt{J}}
\newcommand{\mtK}{\Mt{K}}
\newcommand{\mtL}{\Mt{L}}
\newcommand{\mtM}{\Mt{M}}
\newcommand{\mtN}{\Mt{N}}
\newcommand{\mtO}{\Mt{P}}
\newcommand{\mtP}{\Mt{P}}
\newcommand{\mtQ}{\Mt{Q}}
\newcommand{\mtR}{\Mt{R}}
\newcommand{\mtS}{\Mt{S}}
\newcommand{\mtT}{\Mt{T}}
\newcommand{\mtU}{\Mt{U}}
\newcommand{\mtV}{\Mt{V}}
\newcommand{\mtW}{\Mt{W}}
\newcommand{\mtX}{\Mt{X}}
\newcommand{\mtY}{\Mt{Y}}
\newcommand{\mtZ}{\Mt{Z}}
% Special matrices
\newcommand{\mtLambda}{\MtS{\Lambda}}
\newcommand{\mtPhi}{\MtS{\Phi}}
\newcommand{\mtPsi}{\MtS{\Psi}}
\newcommand{\mtSigma}{\MtS{\Sigma}}
\newcommand{\mtGamma}{\MtS{\Gamma}}
\newcommand{\mtXi}{\MtS{\Xi}}
\newcommand{\mtZero}{\Mt{0}}
\newcommand{\mtOne}{\Mt{1}}
\newcommand{\mtUpsilon}{\MtS{\Upsilon}}
\newcommand{\mtOmega}{\MtS{\Omega}}
% Vectors
\newcommand{\vtA}{\Vt{A}}
\newcommand{\vtB}{\Vt{B}}
\newcommand{\vtC}{\Vt{C}}
\newcommand{\vtD}{\Vt{D}}
\newcommand{\vtE}{\Vt{E}}
\newcommand{\vtF}{\Vt{F}}
\newcommand{\vtG}{\Vt{G}}
\newcommand{\vtH}{\Vt{H}}
\newcommand{\vtI}{\Vt{I}}
\newcommand{\vtJ}{\Vt{J}}
\newcommand{\vtK}{\Vt{K}}
\newcommand{\vtL}{\Vt{L}}
\newcommand{\vtM}{\Vt{M}}
\newcommand{\vtN}{\Vt{N}}
\newcommand{\vtO}{\Vt{P}}
\newcommand{\vtP}{\Vt{P}}
\newcommand{\vtQ}{\Vt{Q}}
\newcommand{\vtR}{\Vt{R}}
\newcommand{\vtS}{\Vt{S}}
\newcommand{\vtT}{\Vt{T}}
\newcommand{\vtU}{\Vt{U}}
\newcommand{\vtV}{\Vt{V}}
\newcommand{\vtW}{\Vt{W}}
\newcommand{\vtX}{\Vt{X}}
\newcommand{\vtY}{\Vt{Y}}
\newcommand{\vtZ}{\Vt{Z}}
% Special vectors
\newcommand{\vtAlpha}{\Vt{\boldsymbol{\alpha}}}
\newcommand{\vtBeta}{\Vt{\boldsymbol{\beta}}}
\newcommand{\vtEta}{\Vt{\boldsymbol{\eta}}}
\newcommand{\vtLambda}{\Vt{\boldsymbol{\lambda}}}
\newcommand{\vtMu}{\Vt{\boldsymbol{\mu}}}
\newcommand{\vtNu}{\Vt{\boldsymbol{\nu}}}
\newcommand{\vtOne}{\Vt{1}}
\newcommand{\vtPsi}{\Vt{\boldsymbol{\psi}}}
\newcommand{\vtPi}{\Vt{\boldsymbol{\pi}}}
\newcommand{\vtSigma}{\Vt{\boldsymbol{\sigma}}}
\newcommand{\vtTau}{\Vt{\boldsymbol{\tau}}}
\newcommand{\vtZero}{\Vt{0}}
% Fields
\newcommand{\fdA}{\Field{A}}
\newcommand{\fdB}{\Field{B}}
\newcommand{\fdC}{\Field{C}}
\newcommand{\fdD}{\Field{D}}
\newcommand{\fdE}{\Field{E}}
\newcommand{\fdF}{\Field{F}}
\newcommand{\fdG}{\Field{G}}
\newcommand{\fdH}{\Field{H}}
\newcommand{\fdI}{\Field{I}}
\newcommand{\fdJ}{\Field{J}}
\newcommand{\fdK}{\Field{K}}
\newcommand{\fdL}{\Field{L}}
\newcommand{\fdM}{\Field{M}}
\newcommand{\fdN}{\Field{N}}
\newcommand{\fdO}{\Field{O}}
\newcommand{\fdP}{\Field{P}}
\newcommand{\fdQ}{\Field{Q}}
\newcommand{\fdR}{\Field{R}}
\newcommand{\fdS}{\Field{S}}
\newcommand{\fdT}{\Field{T}}
\newcommand{\fdU}{\Field{U}}
\newcommand{\fdV}{\Field{V}}
\newcommand{\fdW}{\Field{W}}
\newcommand{\fdX}{\Field{X}}
\newcommand{\fdY}{\Field{Y}}
\newcommand{\fdZ}{\Field{Z}}
% Sets
\newcommand{\stA}{\Set{A}}
\newcommand{\stB}{\Set{B}}
\newcommand{\stC}{\Set{C}}
\newcommand{\stD}{\Set{D}}
\newcommand{\stE}{\Set{E}}
\newcommand{\stF}{\Set{F}}
\newcommand{\stG}{\Set{G}}
\newcommand{\stH}{\Set{H}}
\newcommand{\stI}{\Set{I}}
\newcommand{\stJ}{\Set{J}}
\newcommand{\stK}{\Set{K}}
\newcommand{\stL}{\Set{L}}
\newcommand{\stM}{\Set{M}}
\newcommand{\stN}{\Set{N}}
\newcommand{\stO}{\Set{O}}
\newcommand{\stP}{\Set{P}}
\newcommand{\stQ}{\Set{Q}}
\newcommand{\stR}{\Set{R}}
\newcommand{\stS}{\Set{S}}
\newcommand{\stT}{\Set{T}}
\newcommand{\stU}{\Set{U}}
\newcommand{\stV}{\Set{V}}
\newcommand{\stW}{\Set{W}}
\newcommand{\stX}{\Set{X}}
\newcommand{\stY}{\Set{Y}}
\newcommand{\stZ}{\Set{Z}}
% Alias for math fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmZ}{\mathrm{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmz}{\mathrm{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% it
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\itA}{\mathit{A}}
\newcommand{\itB}{\mathit{B}}
\newcommand{\itC}{\mathit{C}}
\newcommand{\itD}{\mathit{D}}
\newcommand{\itE}{\mathit{E}}
\newcommand{\itF}{\mathit{F}}
\newcommand{\itG}{\mathit{G}}
\newcommand{\itH}{\mathit{H}}
\newcommand{\itI}{\mathit{I}}
\newcommand{\itJ}{\mathit{J}}
\newcommand{\itK}{\mathit{K}}
\newcommand{\itL}{\mathit{L}}
\newcommand{\itM}{\mathit{M}}
\newcommand{\itN}{\mathit{N}}
\newcommand{\itO}{\mathit{O}}
\newcommand{\itP}{\mathit{P}}
\newcommand{\itQ}{\mathit{Q}}
\newcommand{\itR}{\mathit{R}}
\newcommand{\itS}{\mathit{S}}
\newcommand{\itT}{\mathit{T}}
\newcommand{\itU}{\mathit{U}}
\newcommand{\itV}{\mathit{V}}
\newcommand{\itW}{\mathit{W}}
\newcommand{\itX}{\mathit{X}}
\newcommand{\itY}{\mathit{Y}}
\newcommand{\itZ}{\mathit{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ita}{\mathit{a}}
\newcommand{\itb}{\mathit{b}}
\newcommand{\itc}{\mathit{c}}
\newcommand{\itd}{\mathit{d}}
\newcommand{\ite}{\mathit{e}}
\newcommand{\itf}{\mathit{f}}
\newcommand{\itg}{\mathit{g}}
\newcommand{\ith}{\mathit{h}}
\newcommand{\iti}{\mathit{i}}
\newcommand{\itj}{\mathit{j}}
\newcommand{\itk}{\mathit{k}}
\newcommand{\itl}{\mathit{l}}
\newcommand{\itm}{\mathit{m}}
\newcommand{\itn}{\mathit{n}}
\newcommand{\ito}{\mathit{o}}
\newcommand{\itp}{\mathit{p}}
\newcommand{\itq}{\mathit{q}}
\newcommand{\itr}{\mathit{r}}
\newcommand{\its}{\mathit{s}}
\newcommand{\itt}{\mathit{t}}
\newcommand{\itu}{\mathit{u}}
\newcommand{\itv}{\mathit{v}}
\newcommand{\itw}{\mathit{w}}
\newcommand{\itx}{\mathit{x}}
\newcommand{\ity}{\mathit{y}}
\newcommand{\itz}{\mathit{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% frak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\fkA}{\mathfrak{A}}
\newcommand{\fkB}{\mathfrak{B}}
\newcommand{\fkC}{\mathfrak{C}}
\newcommand{\fkD}{\mathfrak{D}}
\newcommand{\fkE}{\mathfrak{E}}
\newcommand{\fkF}{\mathfrak{F}}
\newcommand{\fkG}{\mathfrak{G}}
\newcommand{\fkH}{\mathfrak{H}}
\newcommand{\fkI}{\mathfrak{I}}
\newcommand{\fkJ}{\mathfrak{J}}
\newcommand{\fkK}{\mathfrak{K}}
\newcommand{\fkL}{\mathfrak{L}}
\newcommand{\fkM}{\mathfrak{M}}
\newcommand{\fkN}{\mathfrak{N}}
\newcommand{\fkO}{\mathfrak{O}}
\newcommand{\fkP}{\mathfrak{P}}
\newcommand{\fkQ}{\mathfrak{Q}}
\newcommand{\fkR}{\mathfrak{R}}
\newcommand{\fkS}{\mathfrak{S}}
\newcommand{\fkT}{\mathfrak{T}}
\newcommand{\fkU}{\mathfrak{U}}
\newcommand{\fkV}{\mathfrak{V}}
\newcommand{\fkW}{\mathfrak{W}}
\newcommand{\fkX}{\mathfrak{X}}
\newcommand{\fkY}{\mathfrak{Y}}
\newcommand{\fkZ}{\mathfrak{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\fka}{\mathfrak{a}}
\newcommand{\fkb}{\mathfrak{b}}
\newcommand{\fkc}{\mathfrak{c}}
\newcommand{\fkd}{\mathfrak{d}}
\newcommand{\fke}{\mathfrak{e}}
\newcommand{\fkf}{\mathfrak{f}}
\newcommand{\fkg}{\mathfrak{g}}
\newcommand{\fkh}{\mathfrak{h}}
\newcommand{\fki}{\mathfrak{i}}
\newcommand{\fkj}{\mathfrak{j}}
\newcommand{\fkk}{\mathfrak{k}}
\newcommand{\fkl}{\mathfrak{l}}
\newcommand{\fkm}{\mathfrak{m}}
\newcommand{\fkn}{\mathfrak{n}}
\newcommand{\fko}{\mathfrak{o}}
\newcommand{\fkp}{\mathfrak{p}}
\newcommand{\fkq}{\mathfrak{q}}
\newcommand{\fkr}{\mathfrak{r}}
\newcommand{\fks}{\mathfrak{s}}
\newcommand{\fkt}{\mathfrak{t}}
\newcommand{\fku}{\mathfrak{u}}
\newcommand{\fkv}{\mathfrak{v}}
\newcommand{\fkw}{\mathfrak{w}}
\newcommand{\fkx}{\mathfrak{x}}
\newcommand{\fky}{\mathfrak{y}}
\newcommand{\fkz}{\mathfrak{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Eufrak matrices
\newcommand{\mtkA}{\boldsymbol{\fkA}}
\newcommand{\mtkB}{\boldsymbol{\fkB}}
\newcommand{\mtkC}{\boldsymbol{\fkC}}
\newcommand{\mtkD}{\boldsymbol{\fkD}}
\newcommand{\mtkE}{\boldsymbol{\fkE}}
\newcommand{\mtkF}{\boldsymbol{\fkF}}
\newcommand{\mtkG}{\boldsymbol{\fkG}}
\newcommand{\mtkH}{\boldsymbol{\fkH}}
\newcommand{\mtkI}{\boldsymbol{\fkI}}
\newcommand{\mtkJ}{\boldsymbol{\fkJ}}
\newcommand{\mtkK}{\boldsymbol{\fkK}}
\newcommand{\mtkL}{\boldsymbol{\fkL}}
\newcommand{\mtkM}{\boldsymbol{\fkM}}
\newcommand{\mtkN}{\boldsymbol{\fkN}}
\newcommand{\mtkO}{\boldsymbol{\fkO}}
\newcommand{\mtkP}{\boldsymbol{\fkP}}
\newcommand{\mtkQ}{\boldsymbol{\fkQ}}
\newcommand{\mtkR}{\boldsymbol{\fkR}}
\newcommand{\mtkS}{\boldsymbol{\fkS}}
\newcommand{\mtkT}{\boldsymbol{\fkT}}
\newcommand{\mtkU}{\boldsymbol{\fkU}}
\newcommand{\mtkV}{\boldsymbol{\fkV}}
\newcommand{\mtkW}{\boldsymbol{\fkW}}
\newcommand{\mtkX}{\boldsymbol{\fkX}}
\newcommand{\mtkY}{\boldsymbol{\fkY}}
\newcommand{\mtkZ}{\boldsymbol{\fkZ}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ppl
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pplA}{\mathppl{A}}
\newcommand{\pplB}{\mathppl{B}}
\newcommand{\pplC}{\mathppl{C}}
\newcommand{\pplD}{\mathppl{D}}
\newcommand{\pplE}{\mathppl{E}}
\newcommand{\pplF}{\mathppl{F}}
\newcommand{\pplG}{\mathppl{G}}
\newcommand{\pplH}{\mathppl{H}}
\newcommand{\pplI}{\mathppl{I}}
\newcommand{\pplJ}{\mathppl{J}}
\newcommand{\pplK}{\mathppl{K}}
\newcommand{\pplL}{\mathppl{L}}
\newcommand{\pplM}{\mathppl{M}}
\newcommand{\pplN}{\mathppl{N}}
\newcommand{\pplO}{\mathppl{O}}
\newcommand{\pplP}{\mathppl{P}}
\newcommand{\pplQ}{\mathppl{Q}}
\newcommand{\pplR}{\mathppl{R}}
\newcommand{\pplS}{\mathppl{S}}
\newcommand{\pplT}{\mathppl{T}}
\newcommand{\pplU}{\mathppl{U}}
\newcommand{\pplV}{\mathppl{V}}
\newcommand{\pplW}{\mathppl{W}}
\newcommand{\pplX}{\mathppl{X}}
\newcommand{\pplY}{\mathppl{Y}}
\newcommand{\pplZ}{\mathppl{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ppla}{\mathppl{a}}
\newcommand{\pplb}{\mathppl{b}}
\newcommand{\pplc}{\mathppl{c}}
\newcommand{\ppld}{\mathppl{d}}
\newcommand{\pple}{\mathppl{e}}
\newcommand{\pplf}{\mathppl{f}}
\newcommand{\pplg}{\mathppl{g}}
\newcommand{\pplh}{\mathppl{h}}
\newcommand{\ppli}{\mathppl{i}}
\newcommand{\pplj}{\mathppl{j}}
\newcommand{\pplk}{\mathppl{k}}
\newcommand{\ppll}{\mathppl{l}}
\newcommand{\pplm}{\mathppl{m}}
\newcommand{\ppln}{\mathppl{n}}
\newcommand{\pplo}{\mathppl{o}}
\newcommand{\pplp}{\mathppl{p}}
\newcommand{\pplq}{\mathppl{q}}
\newcommand{\pplr}{\mathppl{r}}
\newcommand{\ppls}{\mathppl{s}}
\newcommand{\pplt}{\mathppl{t}}
\newcommand{\pplu}{\mathppl{u}}
\newcommand{\pplv}{\mathppl{v}}
\newcommand{\pplw}{\mathppl{w}}
\newcommand{\pplx}{\mathppl{x}}
\newcommand{\pply}{\mathppl{y}}
\newcommand{\pplz}{\mathppl{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% phv
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\phvA}{\mathphv{A}}
\newcommand{\phvB}{\mathphv{B}}
\newcommand{\phvC}{\mathphv{C}}
\newcommand{\phvD}{\mathphv{D}}
\newcommand{\phvE}{\mathphv{E}}
\newcommand{\phvF}{\mathphv{F}}
\newcommand{\phvG}{\mathphv{G}}
\newcommand{\phvH}{\mathphv{H}}
\newcommand{\phvI}{\mathphv{I}}
\newcommand{\phvJ}{\mathphv{J}}
\newcommand{\phvK}{\mathphv{K}}
\newcommand{\phvL}{\mathphv{L}}
\newcommand{\phvM}{\mathphv{M}}
\newcommand{\phvN}{\mathphv{N}}
\newcommand{\phvO}{\mathphv{O}}
\newcommand{\phvP}{\mathphv{P}}
\newcommand{\phvQ}{\mathphv{Q}}
\newcommand{\phvR}{\mathphv{R}}
\newcommand{\phvS}{\mathphv{S}}
\newcommand{\phvT}{\mathphv{T}}
\newcommand{\phvU}{\mathphv{U}}
\newcommand{\phvV}{\mathphv{V}}
\newcommand{\phvW}{\mathphv{W}}
\newcommand{\phvX}{\mathphv{X}}
\newcommand{\phvY}{\mathphv{Y}}
\newcommand{\phvZ}{\mathphv{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\phva}{\mathphv{a}}
\newcommand{\phvb}{\mathphv{b}}
\newcommand{\phvc}{\mathphv{c}}
\newcommand{\phvd}{\mathphv{d}}
\newcommand{\phve}{\mathphv{e}}
\newcommand{\phvf}{\mathphv{f}}
\newcommand{\phvg}{\mathphv{g}}
\newcommand{\phvh}{\mathphv{h}}
\newcommand{\phvi}{\mathphv{i}}
\newcommand{\phvj}{\mathphv{j}}
\newcommand{\phvk}{\mathphv{k}}
\newcommand{\phvl}{\mathphv{l}}
\newcommand{\phvm}{\mathphv{m}}
\newcommand{\phvn}{\mathphv{n}}
\newcommand{\phvo}{\mathphv{o}}
\newcommand{\phvp}{\mathphv{p}}
\newcommand{\phvq}{\mathphv{q}}
\newcommand{\phvr}{\mathphv{r}}
\newcommand{\phvs}{\mathphv{s}}
\newcommand{\phvt}{\mathphv{t}}
\newcommand{\phvu}{\mathphv{u}}
\newcommand{\phvv}{\mathphv{v}}
\newcommand{\phvw}{\mathphv{w}}
\newcommand{\phvx}{\mathphv{x}}
\newcommand{\phvy}{\mathphv{y}}
\newcommand{\phvz}{\mathphv{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pzc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pzcA}{\mathpzc{A}}
\newcommand{\pzcB}{\mathpzc{B}}
\newcommand{\pzcC}{\mathpzc{C}}
\newcommand{\pzcD}{\mathpzc{D}}
\newcommand{\pzcE}{\mathpzc{E}}
\newcommand{\pzcF}{\mathpzc{F}}
\newcommand{\pzcG}{\mathpzc{G}}
\newcommand{\pzcH}{\mathpzc{H}}
\newcommand{\pzcI}{\mathpzc{I}}
\newcommand{\pzcJ}{\mathpzc{J}}
\newcommand{\pzcK}{\mathpzc{K}}
\newcommand{\pzcL}{\mathpzc{L}}
\newcommand{\pzcM}{\mathpzc{M}}
\newcommand{\pzcN}{\mathpzc{N}}
\newcommand{\pzcO}{\mathpzc{O}}
\newcommand{\pzcP}{\mathpzc{P}}
\newcommand{\pzcQ}{\mathpzc{Q}}
\newcommand{\pzcR}{\mathpzc{R}}
\newcommand{\pzcS}{\mathpzc{S}}
\newcommand{\pzcT}{\mathpzc{T}}
\newcommand{\pzcU}{\mathpzc{U}}
\newcommand{\pzcV}{\mathpzc{V}}
\newcommand{\pzcW}{\mathpzc{W}}
\newcommand{\pzcX}{\mathpzc{X}}
\newcommand{\pzcY}{\mathpzc{Y}}
\newcommand{\pzcZ}{\mathpzc{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pzca}{\mathpzc{a}}
\newcommand{\pzcb}{\mathpzc{b}}
\newcommand{\pzcc}{\mathpzc{c}}
\newcommand{\pzcd}{\mathpzc{d}}
\newcommand{\pzce}{\mathpzc{e}}
\newcommand{\pzcf}{\mathpzc{f}}
\newcommand{\pzcg}{\mathpzc{g}}
\newcommand{\pzch}{\mathpzc{h}}
\newcommand{\pzci}{\mathpzc{i}}
\newcommand{\pzcj}{\mathpzc{j}}
\newcommand{\pzck}{\mathpzc{k}}
\newcommand{\pzcl}{\mathpzc{l}}
\newcommand{\pzcm}{\mathpzc{m}}
\newcommand{\pzcn}{\mathpzc{n}}
\newcommand{\pzco}{\mathpzc{o}}
\newcommand{\pzcp}{\mathpzc{p}}
\newcommand{\pzcq}{\mathpzc{q}}
\newcommand{\pzcr}{\mathpzc{r}}
\newcommand{\pzcs}{\mathpzc{s}}
\newcommand{\pzct}{\mathpzc{t}}
\newcommand{\pzcu}{\mathpzc{u}}
\newcommand{\pzcv}{\mathpzc{v}}
\newcommand{\pzcw}{\mathpzc{w}}
\newcommand{\pzcx}{\mathpzc{x}}
\newcommand{\pzcy}{\mathpzc{y}}
\newcommand{\pzcz}{\mathpzc{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bb
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bba}{\mathbb{a}}
\newcommand{\bbb}{\mathbb{b}}
\newcommand{\bbc}{\mathbb{c}}
\newcommand{\bbd}{\mathbb{d}}
\newcommand{\bbe}{\mathbb{e}}
\newcommand{\bbf}{\mathbb{f}}
\newcommand{\bbg}{\mathbb{g}}
\newcommand{\bbh}{\mathbb{h}}
\newcommand{\bbi}{\mathbb{i}}
\newcommand{\bbj}{\mathbb{j}}
\newcommand{\bbk}{\mathbb{k}}
\newcommand{\bbl}{\mathbb{l}}
\newcommand{\bbm}{\mathbb{m}}
\newcommand{\bbn}{\mathbb{n}}
\newcommand{\bbo}{\mathbb{o}}
\newcommand{\bbp}{\mathbb{p}}
\newcommand{\bbq}{\mathbb{q}}
\newcommand{\bbr}{\mathbb{r}}
\newcommand{\bbs}{\mathbb{s}}
\newcommand{\bbt}{\mathbb{t}}
\newcommand{\bbu}{\mathbb{u}}
\newcommand{\bbv}{\mathbb{v}}
\newcommand{\bbw}{\mathbb{w}}
\newcommand{\bbx}{\mathbb{x}}
\newcommand{\bby}{\mathbb{y}}
\newcommand{\bbz}{\mathbb{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\scA}{\mathscr{A}}
\newcommand{\scB}{\mathscr{B}}
\newcommand{\scC}{\mathscr{C}}
\newcommand{\scD}{\mathscr{D}}
\newcommand{\scE}{\mathscr{E}}
\newcommand{\scF}{\mathscr{F}}
\newcommand{\scG}{\mathscr{G}}
\newcommand{\scH}{\mathscr{H}}
\newcommand{\scI}{\mathscr{I}}
\newcommand{\scJ}{\mathscr{J}}
\newcommand{\scK}{\mathscr{K}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\scM}{\mathscr{M}}
\newcommand{\scN}{\mathscr{N}}
\newcommand{\scO}{\mathscr{O}}
\newcommand{\scP}{\mathscr{P}}
\newcommand{\scQ}{\mathscr{Q}}
\newcommand{\scR}{\mathscr{R}}
\newcommand{\scS}{\mathscr{S}}
\newcommand{\scT}{\mathscr{T}}
\newcommand{\scU}{\mathscr{U}}
\newcommand{\scV}{\mathscr{V}}
\newcommand{\scW}{\mathscr{W}}
\newcommand{\scX}{\mathscr{X}}
\newcommand{\scY}{\mathscr{Y}}
\newcommand{\scZ}{\mathscr{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% txt
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\txtA}{\text{A}}
\newcommand{\txtB}{\text{B}}
\newcommand{\txtC}{\text{C}}
\newcommand{\txtD}{\text{D}}
\newcommand{\txtE}{\text{E}}
\newcommand{\txtF}{\text{F}}
\newcommand{\txtG}{\text{G}}
\newcommand{\txtH}{\text{H}}
\newcommand{\txtI}{\text{I}}
\newcommand{\txtJ}{\text{J}}
\newcommand{\txtK}{\text{K}}
\newcommand{\txtL}{\text{L}}
\newcommand{\txtM}{\text{M}}
\newcommand{\txtN}{\text{N}}
\newcommand{\txtO}{\text{O}}
\newcommand{\txtP}{\text{P}}
\newcommand{\txtQ}{\text{Q}}
\newcommand{\txtR}{\text{R}}
\newcommand{\txtS}{\text{S}}
\newcommand{\txtT}{\text{T}}
\newcommand{\txtU}{\text{U}}
\newcommand{\txtV}{\text{V}}
\newcommand{\txtW}{\text{W}}
\newcommand{\txtX}{\text{X}}
\newcommand{\txtY}{\text{Y}}
\newcommand{\txtZ}{\text{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\txta}{\text{a}}
\newcommand{\txtb}{\text{b}}
\newcommand{\txtc}{\text{c}}
\newcommand{\txtd}{\text{d}}
\newcommand{\txte}{\text{e}}
\newcommand{\txtf}{\text{f}}
\newcommand{\txtg}{\text{g}}
\newcommand{\txth}{\text{h}}
\newcommand{\txti}{\text{i}}
\newcommand{\txtj}{\text{j}}
\newcommand{\txtk}{\text{k}}
\newcommand{\txtl}{\text{l}}
\newcommand{\txtm}{\text{m}}
\newcommand{\txtn}{\text{n}}
\newcommand{\txto}{\text{o}}
\newcommand{\txtp}{\text{p}}
\newcommand{\txtq}{\text{q}}
\newcommand{\txtr}{\text{r}}
\newcommand{\txts}{\text{s}}
\newcommand{\txtt}{\text{t}}
\newcommand{\txtu}{\text{u}}
\newcommand{\txtv}{\text{v}}
\newcommand{\txtw}{\text{w}}
\newcommand{\txtx}{\text{x}}
\newcommand{\txty}{\text{y}}
\newcommand{\txtz}{\text{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tt
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ttA}{\mathtt{A}}
\newcommand{\ttB}{\mathtt{B}}
\newcommand{\ttC}{\mathtt{C}}
\newcommand{\ttD}{\mathtt{D}}
\newcommand{\ttE}{\mathtt{E}}
\newcommand{\ttF}{\mathtt{F}}
\newcommand{\ttG}{\mathtt{G}}
\newcommand{\ttH}{\mathtt{H}}
\newcommand{\ttI}{\mathtt{I}}
\newcommand{\ttJ}{\mathtt{J}}
\newcommand{\ttK}{\mathtt{K}}
\newcommand{\ttL}{\mathtt{L}}
\newcommand{\ttM}{\mathtt{M}}
\newcommand{\ttN}{\mathtt{N}}
\newcommand{\ttO}{\mathtt{O}}
\newcommand{\ttP}{\mathtt{P}}
\newcommand{\ttQ}{\mathtt{Q}}
\newcommand{\ttR}{\mathtt{R}}
\newcommand{\ttS}{\mathtt{S}}
\newcommand{\ttT}{\mathtt{T}}
\newcommand{\ttU}{\mathtt{U}}
\newcommand{\ttV}{\mathtt{V}}
\newcommand{\ttW}{\mathtt{W}}
\newcommand{\ttX}{\mathtt{X}}
\newcommand{\ttY}{\mathtt{Y}}
\newcommand{\ttZ}{\mathtt{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tta}{\mathtt{a}}
\newcommand{\ttb}{\mathtt{b}}
\newcommand{\ttc}{\mathtt{c}}
\newcommand{\ttd}{\mathtt{d}}
\newcommand{\tte}{\mathtt{e}}
\newcommand{\ttf}{\mathtt{f}}
\newcommand{\ttg}{\mathtt{g}}
\newcommand{\tth}{\mathtt{h}}
\newcommand{\tti}{\mathtt{i}}
\newcommand{\ttj}{\mathtt{j}}
\newcommand{\ttk}{\mathtt{k}}
%\newcommand{\ttl}{\mathtt{l}}
\newcommand{\ttm}{\mathtt{m}}
\newcommand{\ttn}{\mathtt{n}}
\newcommand{\tto}{\mathtt{o}}
\newcommand{\ttp}{\mathtt{p}}
\newcommand{\ttq}{\mathtt{q}}
\newcommand{\ttr}{\mathtt{r}}
\newcommand{\tts}{\mathtt{s}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\ttu}{\mathtt{u}}
\newcommand{\ttv}{\mathtt{v}}
\newcommand{\ttw}{\mathtt{w}}
\newcommand{\ttx}{\mathtt{x}}
\newcommand{\tty}{\mathtt{y}}
%\newcommand{\ttz}{\mathtt{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

